A-ULMPM: An Arbitrary Updated Lagrangian Material Point Method for Efficient Simulation of Solids and Fluids

We present an arbitrary updated Lagrangian Material Point Method (A-ULMPM) to alleviate issues, such as the cell-crossing instability and numerical fracture, that plague state of the art Eulerian formulations of MPM, while still allowing for large deformations that arise in fluid simulations. Our proposed framework spans MPM discretizations from total Lagrangian formulations to Eulerian formulations. We design an easy-to-implement physics-based criterion that allows A-ULMPM to update the reference configuration adaptively for measuring physical states including stress, strain, interpolation kernels and their derivatives. For better efficiency and conservation of angular momentum, we further integrate the APIC[Jiang et al. 2015] and MLS-MPM[Hu et al. 2018] formulations in A-ULMPM by augmenting the accuracy of velocity rasterization using both the local velocity and its first-order derivatives. Our theoretical derivations use a nodal discretized Lagrangian, instead of the weak form discretization in MLS-MPM[Hu et al. 2018], and naturally lead to a "modified" MLS-MPM in A-ULMPM, which can recover MLS-MPM using a completely Eulerian formulation. A-ULMPM does not require significant changes to traditional Eulerian formulations of MPM, and is computationally more efficient since it only updates interpolation kernels and their derivatives when large topology changes occur. We present end-to-end 3D simulations of stretching and twisting hyperelastic solids, splashing liquids, and multi-material interactions with large deformations to demonstrate the efficacy of our novel A-ULMPM framework.

==> tex_input/A_UL_nodal_discretization.tex <==
\section{$A$-ULMPM Formulation for Discrete Systems}
\label{sec:A_UL_nodal}

We now discretize the arbitrary updated Lagrangian formulation described in Section~\ref{sec:arbitrary-updated-lagrangian}. A similar derivation of a total Lagrangian formulation for thermoelasticity was given in~\cite{Xue:2019:NL_L}.  
We use particles to track material information. Below we describe a general discretization methodology, which can either be implemented in pure particle-based discretizations such as SPH~\cite{Desbrun:1996:SPH} or MPM~\cite{jiang2016material}.

The continuum body is considered to be divided into a $N_{\text{dim}}$-dimensional Euclidean space ($\mathbb{E}^N_{\text{dim}}$), in which $N_{\text{dim}}$ denotes the number of dimensions due to spatial discretization, for the purpose of generality, we use \emph{nodes} to discretize the continuum body. These nodes can be particles in pure particle-based methods, such as Smoothed Particle Hydrodynamics(SPH)~\cite{Desbrun:1996:SPH} and grids in pure grid-based methods, such as finite difference method (FDM). Define $i$th node's position vector as $\bs{q}_i$ and its volume as $V_i$. 
We interpolate the Lagrangian of $i$ node at time instant $t_n$ ($\f{L}_i^n$) by its neighboring nodes $j$ at configuration at $t_s$ as follows
\begin{eqnarray}
    \f{L}_i^n=\sum_j \left[\frac{1}{2}\rho_j^0 (\bs{\dot{q}}_j^n)^T\bs{\dot{q}}^n_j -\Psi(\bs{F}_j^{0n})\right]W_{ij}^s V_j^s
    \label{eq:nodal_L}
\end{eqnarray}
We substitute $\f{L}_i^n$ to equation~\eqref{eq:lagrangian} and equation~\eqref{eq:AUL} and get
\begin{enumerate}
\item Kinetic term:
\begin{eqnarray}
     \frac{d}{dt}\left(\frac{\p \f{L}_i^n}{\p \bs{\dot{q}}_i^n}\right)=\sum_j \rho_j^0 \bs{\dot{q}}_j^n W_{ij}^s V_j^s =\sum_j \rho_j^0  W_{ij}^s V_j^s\bs{\ddot{q}}_i^n
\end{eqnarray}
\item Deformation term:
\begin{eqnarray}
    \frac{\p \f{L}_i^n}{\p \bs{q}_i^n}=-\sum_j \frac{\p \Psi(\bs{F}_j^{0n})}{\p\bs{q}_i^n} W_{ij}^s V_j^s= 
    -\sum_j\mathbb{P}_j^{s}  \frac{\p (\bs{F}_j^{sn})^T}{\p \bs{q}_i^s} W_{ij}^s V_j^ss
\label{eq:defromation}
\end{eqnarray}
where $\mathbb{P}_j^s=\mathbb{P}_j^0(\bs{F}_j^{0s})^T/J_j^{0s}$. 
\end{enumerate}
The equation motion of node $i$ at $t_n$ is given by
\begin{equation}
    \sum_j \rho_j^n  W_{ij}^s V_j^s\bs{\ddot{q}}_i^n+\sum_j\mathbb{P}_j^s(\bs{F}_j^{0s})^T  \frac{\p (\bs{F}_j^{0s})^T}{\p \bs{q}_i^s} W_{ij}^s V_j^s=\bs{0}
    \label{eq:dis_L_eq}
\end{equation}
One may have noticed that a further explicit expression of equation~\eqref{eq:dis_L_eq} relies on the concrete formulation of $\bs{F}_j^{0s}$.

\subsubsection{MLS-based gradient operator}
We introduce a MLS-based gradient operator in~\cite{Xue:2019:NL_L} (See Appendix A) that locally minimizes the error of a certain position over its neighboring regime.  
Following the same notation in equation~\eqref{eq:dis_L_eq}, deformation gradient of $j$th node at time instant $t_n$ with respect to an arbitrary configuration (reference configuration) at $t_s$ are given by
\begin{eqnarray}
    \bs{F}_j^{sn}=\left(\sum_{k}(\bs{q}_k^n-\bs{q}_j^n)\otimes \bs{r}_{jk}^s W_{jk}^s V_k^s\right)\left(\sum_{j}\bs{r}_{jk}^s\otimes\bs{r}_{jk}^s W_{jk}^s V_k^s \right)^{-1}
\label{eq:gradient_qp_0s}
\end{eqnarray}
where $k$ represents nodes within the neighboring regime of center node $j$ and $\bs{r}_{jk}^s=\bs{q}_j^s-\bs{q}_j^s$.
\subsubsection{Derivation of $\bs{F}_j^{sn}$}
Based on equation~\eqref{eq:dFdq} in Appendix A, We further evaluate the derivation of $\bs{F}_j^{sn}$ with respect to $\bs{q}_i^s$. 
\begin{eqnarray}
 \frac{\p \bs{F}_j^{sn}}{\p\bs{q}_i^s}=\left[\sum_{k}\left(\delta_{ik}^n-\delta_{ji}^n\right)\otimes \bs{r}_{jk}^s W_{jk}^s V_k^s \right]\left[\sum_{k}\bs{r}_{jk}^s\otimes \bs{r}_{jk}^s W_{jk}^s V_k^s \right]^{-1}
 \label{eq:dFjdqi}
\end{eqnarray}
\subsubsection{Equation of Motion with Arbitrary Updated Lagrangian}
Substituting equation~\eqref{eq:dFjdqi} to equation~\eqref{eq:dis_L_eq} yields the following equation of motion of node $i$ at $t_n$ 
\begin{equation}
\sum_j \rho_j^s  W_{ij}^s V_j^s\bs{\ddot{q}}_i^n+
\sum_j\left[\mathbb{P}_j^s\mathbb{K}_j^s+\mathbb{P}_i^s\mathbb{K}_i^s\right]\bs{r}_{ij}^s W_{ij}^s V_j^s=\bs{0}
\label{eq:EOM1}
\vspace{-3mm}
\end{equation}
where $\mathbb{K}_j^s=\left[\sum_{k}\bs{r}_{jk}^s\otimes \bs{r}_{jk}^s W_{jk}^s V_k^s \right]^{-1}$. We take advantage of $V_j^s=J_i^sV_j^0$ and $\rho_j^s=\rho_0/J_s$ and equation~\eqref{eq:EOM1} can be rewritten by
\begin{eqnarray}
\sum_j \rho_j^0  W_{ij}^s V_j^0\bs{\ddot{q}}_i^n+
\sum_j\left[\mathbb{P}_j^0(\bs{F}_j^{0s})^T\mathbb{K}_j^s+\mathbb{P}_i^0(\bs{F}_i^{0s})^T\mathbb{K}_i^s\right]\bs{r}_{ij}^s W_{ij}^s V_j^0=\bs{0}
\label{eq:EOM2}
\vspace{-3mm}
\end{eqnarray}
Equation~\eqref{eq:EOM2} unifies a general discretization formulation that allows to introduce arbitrarily intermediate configuration $\bs{F}_{0s}$ spanning from total Lagrangian formulation to updated Lagrangian formulations in a nodal discretized system. 
Specifically, we have
\begin{enumerate}
    \item Total Lagrangian formulation: $s=0$ 
\begin{eqnarray}
\sum_j \rho_j^0  W_{ij}^0 V_j^0\bs{\ddot{q}}_i^n+
\sum_j\left(\mathbb{P}_j^0\mathbb{K}_j^0+\mathbb{P}_i^0\mathbb{K}_i^0\right)\bs{r}_{ij}^0W_{ij}^0 V_j^0=\bs{0}
\label{eq:PD_TLSPH}
\end{eqnarray}

\item Eulerian formulation: $s=n$ 

\begin{eqnarray}
\sum_j \rho_j^0  W_{ij}^n V_j^0\bs{\ddot{q}}_i^n+
\sum_j\left[\mathbb{P}_j^0(\bs{F}_j^{0n})^T\mathbb{K}_j^n+\mathbb{P}_i^0(\bs{F}_i^{0n})^T\mathbb{K}_i^n\right]\bs{r}_{ij}^n W_{ij}^n V_j^0=\bs{0}
\label{eq:co_SPH}
\end{eqnarray}
\end{enumerate}
There is no need to update $W_{ij}$, $\bs{r}_{ij}$ and $\bs{K}$ matrices in equation~\eqref{eq:PD_TLSPH}, while they have to be updated at each time step in equation~\eqref{eq:co_SPH}. In comparison with pure particle-based discretization methods, equation~\eqref{eq:PD_TLSPH} recovers state-based Peridynamcis~\cite{Javili:2019:PD, Xue:2018:PD} and Total Lagrangian SPH~\cite{Ganzenmuller:2015:Similarity}, while equation~\eqref{eq:co_SPH} is the associated Eulerian formulation with respect to equation~\eqref{eq:PD_TLSPH} and recovers the correct SPH method~\cite{Vidal:2007:Stabilized}, where the stress term ($\mathbf{P}\bs{F}^T$) was replaced by Cauchy stress. 
The above formulations are derived based on a pure nodal discretization so that equation~\eqref{eq:EOM2} can be directly used for systems discretizated by particles. 
However, neighbouring particle searching is still needed whenever there is a need to update $W_{ij}$, $\bs{r}_{ij}$, and $\mathbb{K}$ matrices. 
The specific discussions regarding pure particle-based methods are outside the scope of this paper. 

